Plasma Cash: Towards more efficient Plasma constructions

Plasma is a framework for scalable off-chain computation. We describe and evaluate Plasma Cash, an improved Plasma construction which leverages non-fungible tokens and Sparse Merkle Trees to reduce the data storage and bandwidth requirements for users. We analyze the cryptoeconomic exit and challenge mechanisms used to keep user funds secured, even when the Plasma Cash chain's consensus algorithm is compromised. A reference implementation is provided for evaluation. Finally, we briefly discuss further improvements that can be made to the Plasma Cash protocol such as arbitrary denomination payments, less user data checking, fast and optimistic exits.

==> protocols/prot_exit.tex <==
\begin{figure}
\begin{minipage}{\columnwidth}
\begin{framed}
    \centering { \bf A coin's state machine and the exit game. \\ Each coin has: $(s, T, c)$} for its state, maturity period, and challenge count. A coin can only be withdrawn when it is in state $q_c$. $T$ is a security parameter which represents the \textit{challenge period}. $now$ represents the current timestamp. \\ Each included transaction (itxn) is of the form (blockNumber, proof, tx). \\ itx.Sender is the address recovered from the signature on the hash of itx.tx.
%\small


    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm,
        semithick]
        \tikzstyle{every state}=[fill=none,draw=black,text=black]

        \node[initial,state] (A)                    {$q_a$};
        \node[state]         (B) [right of=A] {$q_b$};
        \node[accepting,state]         (C) [right of=B]       {$q_c$};

        \path 
        (A) edge [bend left=45]  node {E} (B)
        (B) edge [bend left=45]  node {C} (A)
        (B) edge [loop below] node {IC/R} (B)
        (B) edge              node {F} (C)
        (C) edge [bend left=65]             node {W} (A);
    \end{tikzpicture}

    \begin{enumerate}
        \item StartExit (E) $(pitx, itx): (q_a, 0, 0) \rightarrow (q_b, T, 0)$. Require $pitx.blockNumber < itx.blockNumber$. Store:
            \begin{enumerate}
                \item $eBlk: itx.blockNumber$
                \item $epBlk: pitx.blockNumber$
                \item $eOwner: itx.newOwner$
                \item $epOwner: pitx.newOwner$
            \end{enumerate}
        \item Challenge (C) $(itx): (q_b, T, c) \rightarrow (q_a, 0, 0)$
            \begin{enumerate}
                \item SpentCoin \textit{(challenge with a direct spend of the exiting transaction)}: $(itx.blockNumber > eBlk) \cap (itx.Sender = eOwner)$
                \item DoubleSpend (\textit{challenge with a direct spend of the parent transaction)}: $(epBlk < itx.blockNumber \leq eBlk) \cap (itx.Sender = epOwner)$ 

            \end{enumerate}
        \item Interactive Challenge (IC) $(itx)$: (\textit{challenge with a transaction before the exit}). Require $(itx.blockNumber < epBlk) \cap (now < T/2): (q_b, T, c) \rightarrow (q_b, T, c+1)$. Store: 
            \begin{enumerate}
                \item $cOwner: itx.newOwner$ 
                \item $cBlk: itx.blockNumber$ 
            \end{enumerate}
        \item Respond (R) $(itx):$ \textit{(respond with a direct spend of the challenge transaction)}: $cBlk < itx.blockNumber \leq epBlk \cap itx.Sender = cOwner. (q_b, T, c) \rightarrow (q_b, T, c-1)$
        \item Finalize (F): Requires $now > T$. $(q_b, T, 0) \rightarrow (q_c, T, 0)$
        \item Withdraw (W): $(q_c, T, 0) \rightarrow (q_a, 0, 0)$
    \end{enumerate}

\end{framed}
\end{minipage}
\caption{The basic exit game for a coin}
\label{fig:transfer_coin}
\end{figure}

